Lay-it-out: Interactive Design of Layout-Sensitive Grammars

Layout-sensitive grammars have been adopted in many modern programming languages. However, tool support for this kind of grammars still remains limited and immature. In this paper, we present Lay-it-out, an interactive framework for layout-sensitive grammar design. Beginning with a user-defined ambiguous grammar, our framework refines it by synthesizing layout constraints through user interaction. For ease of interaction, a shortest nonempty ambiguous sentence (if exists) is automatically generated by our bounded ambiguity checker via SMT solving. The soundness and completeness of our SMT encoding are mechanized in the Coq proof assistant. Case studies on real grammars, including a full grammar, demonstrate the practicality and scalability of our approach.

==> tikz/framework.tex <==
\tikzstyle{decision} = [diamond, fill=blue!20, text centered, aspect=2]
\tikzstyle{io} = [rectangle, text centered, text width=7em, fill=green!20]
\tikzstyle{proc} = [rectangle, fill=blue!20, text width=7em, text centered, rounded corners]
\tikzstyle{entity} = [text centered, text width=8em, fill=red!20]
\tikzstyle{line} = [draw, -latex']

\begin{tikzpicture}
    % Place nodes
    % \node [entity] (user) {user};
    \node [io] (grammar) {(layout-sensitive) grammar};
    \node [decision, below=of grammar] (ambig) {SMT solver:\\ambiguous?};
    \node [below left=.5 and .5 of ambig] (stop) {done};
%    \node [proc, below=of ambig] (gen) {word generator};
%    \node [proc, below=of gen] (parser) {GLL parser};
    \node [proc, below=of ambig] (gen) {decode\\ ambiguous word\\ from model};
    \node [proc, right=.15 of ambig] (synt) {grammar refinement};
%    \node [entity, right=4.3 of parser] (select) {parse tree selection};
    \node [entity, right=2.5 of gen] (select) {user interaction (word formatting)};
    \node [entity, right=2.5 of grammar] (input) {initial grammar};
    \node [below=.25 of select, red] {user};
    % Draw edges
    \path [line, red, thick] (input) -- node [above] {input} (grammar);
    \path [line] (grammar) -- node [left] {preprocess \& \\encode} (ambig);
    \path [line] (ambig.west) -| node [left] {no} (stop);
    \path [line] (ambig) -- node {yes} (gen);
%    \path [line] (gen) -- node {word} (parser);
%    \path [line, dashed] (parser.east) to [bend right=45] node [right] {not ambiguous} (gen.east);
%    \path [line] (parser) -- node [below] {ambiguous word \& \\ parse trees} (select);
    \path [line] (gen) -- node [below] {ambiguous word \& \\ parse trees} (select);
    \path [line, red, thick] (select) -- node {feedback} (synt);
    \path [line] (synt) -- node [right] {add layout \\ \qquad restrictions} (grammar);
    % Draw user rectangle
    \draw[red, thick, dashed, rounded corners]
        ($(select.south east)+(.2,-.2)$) rectangle ($(input.north west)+(-.2,.2)$);
\end{tikzpicture}

